Expressive Communication: A Common Framework for Evaluating Developments in Generative Models and Steering Interfaces

There is an increasing interest from ML and HCI communities in empowering creators with better generative models and more intuitive interfaces with which to control them. In music, ML researchers have focused on training models capable of generating pieces with increasing long-range structure and musical coherence, while HCI researchers have separately focused on designing steering interfaces that support user control and ownership. In this study, we investigate through a common framework how developments in both models and user interfaces are important for empowering co-creation where the goal is to create music that communicates particular imagery or ideas (e.g., as is common for other purposeful tasks in music creation like establishing mood or creating accompanying music for another media). Our study is distinguished in that it measures communication through both composer's self-reported experiences, and how listeners evaluate this communication through the music. In an evaluation study with 26 composers creating 100+ pieces of music and listeners providing 1000+ head-to-head comparisons, we find that more expressive models and more steerable interfaces are important and complementary ways to make a difference in composers communicating through music and supporting their creative empowerment.

==> scratchpad.tex <==
%%%%% START COMMENTING OUT QUAL RESULTS
\if 0
\section{Qualitative Results}

\subsection{Experiences Composing with Different Interfaces}

\subsubsection{Steering Interfaces Supported Creative Empowerment}
% First, talk more generally about the comparison, and why more ways to provide input and make decisions in the process is helpful.
% Then, describe how chunk-by-chunk supports thinking about flow and progression in the piece
% Then, describe how semantic dimensions helps here.  Add specifics like how many primitives aligned with how they thought about things. And that others like "key change relative to last chunk" was useful modulation.

Overall, participants using the Steering Interface had a much stronger sense of control. They felt there were many more ways to provide input to how the music would sound, and several places where they could make decision during the process.  In contrast, composers using the Radio interface felt they only had only a single means of influencing the output, which was choosing. % How did they feel? What was their explanation (mostly just choosing?)
Several participants emphasized how they did not feel like they were composing or collaborating, but rather described their role as a listener and evaluator.

Participants using the Steering interface felt they had the ability to make several decisions for each chunk. As a result, they felt control over how the piece would progress. 
% How did they feel, composing? 
For example, P7 mentioned that ``With the Steering Interface, I could more piece it together, think more about the direction it takes.  It helped me composing a flow, a narrative.'' 
% Why is that? Generally because they had more ability to provide input? Fine grain allowed them to tell a story, form the shape, had room to think about these things?


% -- Say something about sometimes when by chance it matched the idea they had in their head, they felt much more ownership
% -- Say something about being able to find multiple samples that could meet their musical goals.

\subsubsection{Limits to Steering using Semantic Dimensions}
While the Chunks provided more ways to steer the generated output, users described two core limitations that prevented them from feeling a maximum amount of control and ownership, including (1) mismatches between parameter settings and actual outputs; and (2) lack of direct manipulation.   First, users struggled when there was a mismatch between the parameter settings for constraining the generated outputs and the actual generated outputs they heard. 
%This could happen if the set of pre-generated samples did not have samples that met the requested criteria. 
For example, while a user might request for the model to generate music that is "very slow, very low, very many pitches, and dissonant", the generated outputs could sometimes might not be as "dissonant" as they user would have expected.  This led to users feeling that the Steering Interface sometimes provided a "false sense of control", and that they would often resort to just generating random samples.  
% This challenge is due to a limitation in how a rejection sampling approach works for constrained generated outputs.
Second, users felt they could not feel a full sense of ownership over the piece when they had never chose the individual notes, or played an instrument as input to the generation. In this case, users felt that the option to directly manipulate any notes was critical to them feeling they had ownership. One participant described how using the chunks and steering interface felt like they were ``a film director that's working with a composer that knows a lot more about music than I do. I am influencing the end results, but I am not sure if it's actually true. I feel like the computer has more control that I do'' (P10).


\subsubsection{Relinquishing control to support exploration of new ideas}
% With Radio, because they were forced to listen and only curate options that match, people sometimes discovered samples that achieved the expression of the card, but in a different way than they initially thought.
While the Steering Interface did provide specific ways to control the direction, several participants felt they could still use the Radio Interface to find a musical phrase that expressed the musical goals equally as well. 
% Bring in counts stats on how many participants rated the Interface Comparison equally? 
Several participants were open-minded to the model generating musical outputs that surprised them and was different than their initial expectations. For example, P15 said ``I was surprised by the random composition, taking it into a musical direction that I would have otherwise gone... this tool makes me go beyond my first idea, giving ideas that help one express an idea in a different way.''
% Add YUM's perspective on not being too much of a control freak in a collaboration.
% IMPLICATION

\subsubsection{Efficacy in Expression allows for considerations of Musical Coherence}
When selecting chunks, creators often kept in mind musical coherence, how the transitions worked across chunks, and how the piece ended.  In some cases, people were targeting musical coherence. For MusicTransformer, however, much of its samples are musically coherent (see the comparison between MusicTransformer and PerformanceRNN).
So many of the Radio samples did have coherence. For the final option creators chose with the radio, they sometimes had several options to choose from, and would factor in musicality and coherence into this final decision.  

\subsubsection{Importance of Establishing a First Chunk to Seed Continuations} % 
Many people using the Steering Interface said that they could find multiple musical phrases that matched their expressive and musical goals.  Finding a first chunk that captured the general mood and tempo helped made them feel like they were already close to communicating the imagery and ideas of the card.  From there, several composers felt comfortable letting the AI generate random continuations in the second and third chunk because they were confident that they had set a good initial direction. These participants mentioned that because many of the generated continuations in subsequent chunks continued the express the same feeling established by the first chunk, they had more flexibility to tailor the music in each subsequent chunks based more personal tastes and what might make the composition more musical and coherent.  For example, many participants when composing the last chunk felt it was important to provide a ending that resolved the musical phrase, and so chose the option that primarily satisfied this goal.

However, participants who did not establish a first chunk that strongly matched the mood of the card could often struggled to find continuations in subsequent chunks that achieved their musical goals.  In our studies, we observed composers not establishing a first chunk in two different scenarios. First, some participants could not find a great option for the first chunk and instead had to opt for something that is satisfactory (e.g., the slow tempo was appropriate for peaceful and dreamy, but contained too much dissonance for their tastes).  Second, we observed participants that were overly hopeful that the first chunk was open-ended enough to allow for steering subsequently generated chunks to express all the imagery and words of the card.  When the first chunk did not strongly match the mood, participants could still struggle to find generated continuations that shifted the later chunks in their desired direction.  This illustrates how it can be challenging to implement steering interfaces for changing the direction of the generation when the model's default nature is to repeat and elaborate on musical themes. In the case of our implementation of the steering capabilities, which is relies on a filtering or rejection based sampling approach, it can be entirely possible that a fixed size set of pre-generated continuations may not contain a sample that changes the musical qualities (e.g., tempo, pitch, dissonance) so much from the first. 
% Future Direction: A little sense of the diversity of the children -- this could correct assumptions where people are constraining themselves too much by choosing some parents over others. This could still be useful, even if we used a conditional-model in the backend, since these conditional models can suffer tradeoffs in "likelihood" and going "off distribution". 
 
% \subsubsection{Supporting musical expression when the clarity of the goals evolve}
%\subsubsection{Using Random Generation vs Constraining the Generation along Semantic Dimensions}
% or goals evolving?
%How goals evolved, and how different interfaces supported achieving the goals as they evolved.
% With the chunks, they felt they could achieve because they would mostly enact the ways they imagined the music (by using the steering dimensions).
% When they didn’t have something specific in mind, they would randomly generate chunks. Once they heard that, it would give a very clear theme or imagery for how the rest of the chunks should go.


\subsection{Experiences Composing with Different Models}

% Signposting

% Advantages and Disadvantages of Predictability, Repetition, and Coherence
% 
\subsubsection{Advantages and Disadvantages of Predictability, Repetition, and Coherence} 
Participants began to form their own impressions of each model after generating multiple generated samples from each model. The pretrained MusicTransformer model generated samples that had more musical coherence.  Participants felt that this model continued and built upon a theme more effectively and communicated a "single thread" of an idea. MusicTransformer's ability to maintain a ``coherent thread'' of a musical idea helped with painting a clear image of a scene. Many participants felt that MusicTransformer was especially useful for expressing imagery and ideas such  ``dreamy'', ``curiosity'', ``reflective'', ``melancholy'', ``easy going'', and ``satisfied''. In contrast, With the PerformanceRNN model, participants often found that only parts of the full 15 second phrase could apply to the cards, but when the piece would change musical ideas, it rendered it less usable.

Participants had a split opinion on whether the predictable, repetitive nature of the music generated with MusicTransformer helped with communicating other ideas like “stuck” and “creeping”. 
Some found that the repetition, helped them when trying to express feelings of “stuck” (“since the phrase goes up but then ultimately returns to the same note, it has this feeling of being stuck”) and “creeping” (“the tense, [long] repeated chord built up this feeling of tenseness”).
However, several participants felt that MusicTransformer's generated outputs could be "too steady", which was less likely to evoke the feeling of being "uncomfortable and creepy" or a scene of "a comparison with a climax".  For example, a participant who wanted to create music that expressed “creeping” could not find a satisfactory phrase based on the 10 options generated by MusicTransformer. They commented that desired music that PerformanceRNN might produce, so as to leverage the unpredictable rhythms of “long short notes that makes the listener uncomfortable, and thus expresses the creepy idea.”

\subsubsection{Advantages and Disadvantages of Unexpectedness and Diversity}
Several participants appreciated the surprise and variety that PerformanceRNN produced.
For example, P13 said that PerformanceRNN ``varied more greatly.  Yes, some pieces have [less desirable] pauses in between. But when it works, it has something that others don't. With [MusicTransformer], it is very safe, and lots of the pieces are similar. If you look at the card, each of them are different. So, you need the music to be different too.''  With the model comparison, both systems had a radio interface where composers would need to curate the best from a set of randomly generated options. So, some participants highlighted how the diversity in the options allowed them to find an example that worked well for any of the different cards which spanned the spectrum of moods and energy.

% \subsubsection{Coherence as a Musical Quality Thing}
% If it has more musical quality, then more of the samples are actually usable (they won't be thrown away for quality first).

\subsubsection{Influence of the Cultural-Relatedness of the Music Training Data}
% Music that is more relatable -- things they've heard in movies, in video games, in modern music, makes it easier to attach a context/mood to them.
Participants felt that the Music Transformer model tended to generate more modern music or pop-songs which were easier for them relate to.  For example, composers sometimes would connect a certain music to a particular cultural reference, such as reminders to specific songs they have heard (e.g., ``it sounds very similar to the song `Silent Night', so I already imagine snow and winter'') and types of music they have heard used in specific contexts (e.g., ``this is music that plays at the beginning of a Japanese anime drama''; ``it reminds me of the music that plays during a boss battle in a video game''). They could use these connections to other contexts to guide their decision on whether this music expressed the matching imagery or words of the cards.  In contrast, participants noticed that the PerformanceRNN model would generate music that associated with classical music, or a 20th century modern style.  Several participants noted that these pieces did not express something that was clearly evocative. Nonetheless, they used musical dimensions such as a tempo, density of notes, and dissonance to discern which musical pieces might match the words in a card.

% Bias towards music they like to listen to, to their preference







\subsection{Reflections about the Expressive Communication game}

\subsubsection{Purposeful Expression Task Guides the Composer Experience}
Participants felt that having a purposeful task helped them have a clearer direction and more effectively discern AI generated outputs.
For example, P4 said ``It gives good guidance on what I am aiming for in the music options.  It gives a good center for what I'm looking for with the AI generated options. Rather than just listening to the music without a goal, and me saying “This is fine!”, having a card with end goal helped me better judge different AI tools.’’ Since the Expressive Communication framework gives composers several musical goals to capture, they are able to to focus on strategies for expressing the mood with the steering interface, or listening and evaluating the outputs on this focused dimension for the Model Interface. As one participant mentioned, the Expressive Communication game ``gives good guidance on what I am aiming for in the music options. Rather than just listening to the music without a goal, and me saying [the AI generated music] sounds good, having a card with end goal helped me better judge different AI tools.''

\subsubsection{Creativity under Constraints}
While the task was assigned to composers, participants also commented how the expressive communication task still left room for their imagination and creativity. 
For example, P7 said ``Composing for cards is extremely for focused -- it gives you a mood, gives you a pace and tempo.  With your imagination with what happens in the imagery of the card, you can think of a direction where the mood goes.''

Moreover, when composers had multiple options that could match a given mood and tempo, they also would focus on composing music that matched their own musical taste. One composer thought of it as ``finding the balance of writing music, that's easy for people to guess [the feeling of the card], and that's interesting. For easy to guess, your best bet is to go for the most cliche. Fits the mental model of what people think --- the expected. Then, creating something that musically interesting.''.  This composer went on to say that they aspired to be like composers who ``compose music for a film'' who both write something appropriate for the mood and ``who can deliver it to listeners in new and surprising ways'' (P10).
\fi 
%%%%% END COMMENTING OUT QUAL RESULTS


%%% Discussion Scratch
Some of the most surprising challenges users faced included (1) mismatches in the settings and how the outputs actually sounded (e.g., not as dissonant as they had thought); (2) an optimistic (but sometimes misfounded) belief they could make subsequent chunks have important qualities, and a lack of ability to backtrack quickly; (3) users often reflect on all the possible parameters, and more likely will set many of them; (4) since users will often specify many constraints on the generation, there efforts can lack exploration; (5) when constraining the generation via the semantic parameters, the generated samples can lack diversity and may not capture their goals well; (7) when using chunks, it can be hard to effectively judge whether the piece can work for 5 seconds; (10)


% Surprising desires
 (9) some were willing to have some incoherence if it meant that the samples it generated were more diverse or unique -- participants expressed wanting to have the ability to have the best of both models. "MusicTransformer is traditional, safe, and would be too limiting, while PerformanceRNN would not fit all the use cases"
 % is too would help (sort of like conventional vs surprising or raising the temperature);

% Useful ideas for future use cases
Creating a seed of an idea that can be used for manual composing.  AI is really good at generating lots of content, and then real composers can continue off of that seed.
Having many more types of control knobs, for it to really feel like it's quite a unique part of the parameter space someone is in.
Being able to control the amount of chunks a piece should be, and really getting it to be like a 10 chunks piece.

% Observations or tradeoffs
(6) when choosing chunks, they try to use more local features to tell a story of moods (e.g., increased tempo to indicate intensity, shift in key to surprise the reader) where as with longer phrases, they can focus on ideas for more global features of the phrase (e.g., is it all the right tempo? does the whole piece have a dissonant tone?);
% Interface Challenges
